Inducing Equilibria in Networked Public Goods Games through Network Structure Modification

Networked public goods games model scenarios in which self-interested agents decide whether or how much to invest in an action that benefits not only themselves, but also their network neighbors. Examples include vaccination, security investment, and crime reporting. While every agent's utility is increasing in their neighbors' joint investment, the specific form can vary widely depending on the scenario. A principal, such as a policymaker, may wish to induce large investment from the agents. Besides direct incentives, an important lever here is the network structure itself: by adding and removing edges, for example, through community meetings, the principal can change the nature of the utility functions, resulting in different, and perhaps socially preferable, equilibrium outcomes. We initiate an algorithmic study of targeted network modifications with the goal of inducing equilibria of a particular form. We study this question for a variety of equilibrium forms (induce all agents to invest, at least a given set $S$, exactly a given set $S$, at least $k$ agents), and for a variety of utility functions. While we show that the problem is NP-complete for a number of these scenarios, we exhibit a broad array of scenarios in which the problem can be solved in polynomial time by non-trivial reductions to (minimum-cost) matching problems.

==> section/backup/hard.tex <==
In this section we present hardness results for our problem. We show that a special case of our problem is NP-Complete. The special case is where the $g_i$ is a submodular function. The idea of the proof is by constructing a reduction from the \textit{Max-k-cover} problem.  Suppose the function $g_i$ is defined as the following:
\begin{equation}
g_i(x_i, \mathcal{S}_i) = \begin{cases} \hat{g}_i(\mathcal{S}_i \cup \{i \}), &  x_i = 1 \\ \hat{g}_i(\mathcal{S}_i), & x_i = 0 \end{cases},
\end{equation}
where $\hat{g}_i: 2^{|\mathcal{N}_i|}\rightarrow \mathbb{R}_+$ is a submodular function. A player $i$ chooses to invest \textit{iff} $U_i(1, \mathcal{S}_i) \ge U_i(0, \mathcal{S}_i)$, which is equivalent to the following condition:
\begin{equation}\label{eq:iff_sub}
\underbrace{\hat{g}_i(\mathcal{S}_i \cup \{i \}) - \hat{g}_i(\mathcal{S}_i)}_{:=\Delta \hat{g}_i(\mathcal{S}_i)} \ge c_i.
\end{equation}
The function $\Delta \hat{g}_i(\mathcal{S}_i)$ is submodular  due to the submodularity of $\hat{g}_i$. The formal statement of the hardness result is in Theorem~\ref{th:submodular_hard}:
\begin{theorem}\label{th:submodular_hard}
When $g_i(x_i, \mathcal{S}_i)$ is a submodular function of $\mathcal{S}_i$, the problem in Definition~\ref{def:main} is NP-Complete. 
\end{theorem} 
\begin{proof}
First, given a target action profile $\bm{x}^{\ast}$ we can check if it is a PSNE by iteratively checking if  Eq.~\eqref{eq:iff_sub} holds (not holds) for every investor (non-investor), which takes polynomial time. Next, we construct a reduction from the \textit{Max-k-cover} problem. Given a ground set $\mathcal{U}$, a set of subsets $\mathcal{A} = \{ A_1, A_2, \dots, A_m \,|\, \forall i: A_i\subseteq \mathcal{U} \}$, and an integer $k$, the objective of the \textit{Max-k-cover} problem is to find a subset $\mathcal{A}^\prime \subseteq \mathcal{A}$ such that $|\mathcal{A}^\prime| \le k$ and the number of covered elements $\big| \cup_{A_i \in \mathcal{A}^\prime} A_i \big|$ is maximized. We consider the decision version of the \textit{Max-k-cover} problem. Given an integer $m$, the decision version is to determine if the number of covered elements is at least $m$. For any instance  $MaxK(m)$  of the \textit{Max-k-cover} problem we construct an instance of our problem. The first step is to construct a graph $\mathcal{G}=(V, E)$. The node set $V$ consists of $m$ blue nodes and one red node, where each blue node corresponds to a set in $\mathcal{A}$. The edge set $E$ is empty. An example graph with $m=7$ is showed in Figure~\ref{fig:star_graph}. Next, we define the nodes' utility functions. For any blue node we set its  $\hat{g}_i$ as the following submodular function:
\[
\hat{g}_i(X) = |X|,
\]
which returns the cardinality of its argument. In addition, let the cost coefficient of any  blue node satisfy $c_i < 1$.  It is direct to verify that blue nodes always invest. For the red node we define its utility function as the following:
\begin{equation}\label{eq:sub_g}
\Delta \hat{g}_r(\mathcal{S}_r) := \big| \cup_{i \in \mathcal{S}_r} A_i \big|,
\end{equation}
where $\mathcal{S}_r$ is the investors among the red node's neighbors.  The cost coefficient of the red node is set to $c_r=m$, so it invests \textit{iff} $\Delta \hat{g}_r(\mathcal{S}_r) \ge m$.  The budget parameters  are set to $B_1=0$ and $B_2 = k$, which means we can add at most $k$ edges but cannot remove any edge. The setup of the budget parameters indicates that $| \mathcal{S}_r | \le k$. Suppose the target action profile $\bm{x}^{\ast} = \bm{1}$. Since the blue nodes always invest, what remains is to add edges such that the red node invests. Adding an edge to $\mathcal{G}$ is equivalent to choosing a subset from $\mathcal{A}$. If $\bm{x}^\ast$ is realizable, the number of covered elements is at least $m$. So the answer to $MaxK(m)$ is ``yes''. Otherwise the answer is ``no''. In conclusion,  if there were a polynomial-time algorithm to solve our problem then the \textit{Max-k-cover} problem would be polynomial-time solvable. 

\begin{figure}[h]
\centering
\setlength{\tabcolsep}{0.1pt}
\begin{tabular}{c}
\stargraph{7}{2}
\end{tabular}
\caption{An example graph where each blue node corresponds to a set in $\mathcal{A}=\{A_1, \dots, A_7 \}$.}
\label{fig:star_graph}
\end{figure}
\end{proof}

The hardness result for the case where $g_i$ is a supermodular function can be similarly obtained.  The formal statement is  in Theorem~\ref{th:supermodular_hard}. The proof utilizes a similar reduction as the  one we used in the proof of Theorem~\ref{th:submodular_hard}. We defer the proof to the Appendix. 

\begin{theorem}\label{th:supermodular_hard}
When $g_i(x_i, \mathcal{S}_i)$ is a supermodular function, the problem in Definition~\ref{def:main} is NP-Complete. 
\end{theorem}






==> section/backup/hard_general.tex <==
In this section suppose $g_i$ is defined as follow:
\begin{equation}
g_i(x_i, \mathcal{S}_i) = \hat{g}_i(n_i + x_i),
\end{equation}
where $n_i$ is the number of investors among player $i$'s neighbors and  $\hat{g}_i:\mathbb{N}_{\ge 0} \rightarrow \mathbb{R}_+$ is a non-decreasing function.  We have the following hardness result:
\begin{theorem}
Suppose $\hat{g}_i:\mathbb{N}_{\ge 0}\rightarrow \mathbb{R}_+$ is a general non-decreasing function, the problem in Definition~\ref{def:main} is NP-Complete. 
\end{theorem}
\begin{proof}
Given a target action profile $\bm{x}^\ast$ and a modified graph $\hat{\mathcal{G}}$ (after adding or removing edges), we iteratively check if Eq.~\eqref{eq:iff} holds (not holds) for every investor (non-investor), which takes polynomial time. We construct a reduction from the \textit{Hamiltonian Cycle} (HC) problem. Given a graph $\mathcal{G}=(V, E)$, the HC problem asks if there is a Hamiltonian Cycle in $\mathcal{G}$. Let \texttt{HC}($\mathcal{G}$) be an instance of the HC problem. In what follows we construct a graph $\mathcal{G}^\prime$.  We use nodes and players interchangeably. First, we run a Depth-First Search (DFS) on $\mathcal{G}$, which labels each edge  as either \textit{tree edge} or \textit{back edge}. Then for each tree edge $(u, v)$  we add a node $w_{u, v}$ that connects to both $u$ and $v$, which results in $\mathcal{G}^\prime$. An example of $\mathcal{G}^\prime$ is showd in Figure~\ref{fig:gen_g_demo}. The  original graph $\mathcal{G}$ is in blue, which can be thought of as an induced subgraph of $\mathcal{G}^\prime$. The newly added nodes and edges are in red. 
Next, we define the utility functions of the nodes in $\mathcal{G}^\prime$ through a payoff matrix as in Table~\ref{tab:general_g}:
\begin{table}[H]
\centering
\begin{tabular}{lccc}
                       & \multicolumn{1}{l}{$n_i < 2$}   & \multicolumn{1}{l}{$n_i = 2$}   & \multicolumn{1}{l}{$n_i > 2$}   \\ \cline{2-4} 
\multicolumn{1}{l|}{0} & \multicolumn{1}{c|}{$c-2\gamma$}        & \multicolumn{1}{c|}{$c-\gamma$} & \multicolumn{1}{c|}{$c+\gamma$} \\ \cline{2-4} 
\multicolumn{1}{l|}{1} & \multicolumn{1}{c|}{$0$} & \multicolumn{1}{c|}{$c$}        & \multicolumn{1}{c|}{$c$}        \\ \cline{2-4} 
\end{tabular}
\caption{Payoff matrix for the nodes in $\mathcal{G}^\prime$, where $c, \gamma > 0$ and $c > 2\gamma$. }
\label{tab:general_g}
\end{table}
The utility functions resulted from Table~\ref{tab:general_g} satisfy the non-decreasing assumption. From Table~\ref{tab:general_g} we know a player invests \textit{iff} it has exactly two investing neighbors. Let the target action profile $\bm{x}^{\ast}=\bm{1}$, which means all players should invest. The budget parameters are set to $B_1=|E|$ and $B_2=0$, where $|E|$ is the number of blue edges.
This setup indicates that we can remove up to $|E|$ edges but cannot add any edge to $\mathcal{G}^\prime$. Notice that a red node is connected to exactly two investors, so we do not need to remove any red edge. 

We first show that if $\bm{x}^{\ast}$ is realizable on $\mathcal{G}^\prime$ then the graph $\mathcal{G}$ contains a HC. Let $\hat{\mathcal{G}}^\prime$ be the graph resulted from $\mathcal{G}^\prime$ after removing edges. We know $\hat{\mathcal{G}}^\prime$ is a 2-regular graph. We claim that $\hat{\mathcal{G}}^\prime$ is connected, which is proved by induction in what follows. Recall that we  only remove blue edges, which are either \textit{tree edges} or \textit{back edges}. Suppose we remove a back edge $(u, v)$. By definition we know $v$ is an ancestor of $u$.  There must be a path from $v$ to $u$ that is not involving $(u, v)$.  Therefore removing a back edge does not disconnect $\mathcal{G}^\prime$. Removing a tree edge $(x ,y)$ does not disconnect $\mathcal{G}^\prime$ either, since there is a detour $x \rightarrow w_{x, y} \rightarrow y$. Suppose removing $k-1 < |E|$ edges does not disconnect $\mathcal{G}^\prime$. Now we remove one extra edge $(u, v)$, which is either a \textit{tree edge} or a \textit{back edge}. If $(u, v)$ is a \textit{tree edge} then  $\hat{\mathcal{G}}^\prime$ is not disconnected due to the detour $x \rightarrow w_{x, y} \rightarrow y$. If $(u, v)$ is a \textit{back edge} then there exists a  path $P$ (not involving $(u, v)$) from $v$ to $u$ in the original graph $\mathcal{G}$. The path $P$ only consists of \textit{tree edges}. The initially removed $k-1$ edges may contain some of the edges in $P$, however, as we argued before removing any \textit{tree edges} does not disconnect $\mathcal{G}^\prime$ because of their associated detours. Therefore the graph $\hat{\mathcal{G}}^\prime$ after removing $k$ edges is connected. A 2-regular graph contains one or more disconnected cycles. Since we showed that $\hat{\mathcal{G}}^\prime$ is connected, it must be a single cycle. This single cycle is a HC of $\hat{\mathcal{G}}^\prime$. We  identify the HC of the original graph $\mathcal{G}$ by replacing each $x \rightarrow w_{x, y} \rightarrow y$ path in $\hat{\mathcal{G}}^\prime$ with an edge $(x, y)$. In summary, if $\bm{x}^{\ast}$ is realizable on $\hat{\mathcal{G}}^\prime$  then $\mathcal{G}$ contains a Hamiltonian Cycle. 

The other direction is to prove if $\mathcal{G}$ contains a HC then $\bm{x}^{\ast}$ is realizable on $\mathcal{G}^\prime$, in other words, a 2-regular graph $\hat{\mathcal{G}}^\prime$ can be constructed from $\mathcal{G}^\prime$ by removing edges. 

\begin{figure}[H]
\centering
\setlength{\tabcolsep}{0.1pt}
\begin{tabular}{c}
\includegraphics[width=2.4in]{figures/general_g.png} 
\end{tabular}
\caption{An example of graph $\mathcal{G}^\prime$, where the original graph $\mathcal{G}$ contains the blue nodes and edges.}
\label{fig:gen_g_demo}
\end{figure}
\end{proof}

==> section/backup/tractable.tex <==
% \begin{table*}[t!]
% \centering
% \begin{tabular}{@{}lccl@{}}
% \toprule
%                                                             % &                      &                      &                                                         \\ \midrule
% % $\bm{x}^{\ast}$                                             &                      &                      & target action profile                                   \\
% $\mathcal{S}=\{ i | x^{\ast}_i=1 \}$                          &                      &                      & investing players in $\bm{x}^{\ast}$                    \\
% $\mathcal{S}^\prime=\{ i | x^{\ast}_i=0 \}$                                 &                      &                      & non-investing players in $\bm{x}^{\ast}$                \\
% $E^\prime=\{ (u, v) | u \in \mathcal{S}, v \in \mathcal{S}^\prime \}$          & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & edges between investing players and non-investing players            \\
% $d_{\hat{\mathcal{G}}}(i)$               & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &     degree of node $i$ in graph $\mathcal{\hat{G}}$                   \\
% $\mathcal{I}=\{ i | x^{\ast}_i=1 \land d_{\hat{\mathcal{G}}}(i)=0 \}$ & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & investing players with degree zero in $\mathcal{G}^\prime$  \\ 
% $\mathcal{C} = \{ (u, v)  | u, v \in \mathcal{S}^\prime \}$          & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & edges between investing players  \\
% $\mathcal{J}=\{ i | i \in \mathcal{S} \land \big(\mathcal{N}_i \cap \mathcal{S}^\prime =\emptyset \big) \}$          & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & non-investing players that has no investing neighbor  \\ \bottomrule
% \end{tabular}
% \caption{Notations used in Section~\ref{sec:tractable}.}
% \label{tab:notation}
% \end{table*}



Due to the hardness result presented in Section~\ref{sec:hard} we consider two tractable cases where  $g_i$ is either convex or concave. Let $n_i= |\mathcal{S}_i|$, which is the number of investors among player $i$'s neighbors.  Suppose  $g_i$ is defined as follow:
\begin{equation}
g_i(x_i, \mathcal{S}_i) = \hat{g}_i(n_i + x_i),
\end{equation}
where $\hat{g}_i$ is either convex or concave. In addition, $\hat{g}_i$ is a non-decreasing function. In what follows we show that there are polynomial-time algorithms for the tractable cases. We term $\bm{x}^{\ast}$ as \textit{realizable} if it is a PSNE of the BNPG played on the modified graph $\hat{\mathcal{G}}$.



\subsection{Convex $\hat{g}_i$}
Similar to the analysis presented in last section, a player $i$ decides to invest \textit{iff} the following condition holds:
\begin{equation}\label{eq:iff}
\underbrace{\hat{g}_i(1 + n_i) - \hat{g}_i(n_i)}_{:=\Delta \hat{g}_i(n_i)} \ge c_i,
\end{equation}
where $\Delta g_i(n_i)$ is  non-decreasing with respect to $n_i$ due to the convexity of $\hat{g}_i$. Suppose $\forall i: c_i \le \Delta g_i(N-1)$ (otherwise there exists some players that can  never invest). In addition,  $\Delta g_i(n_i)$ can  take at most $N-1$ values. Let $t_i = \Delta g_i^{-1}(c_i)$. Then Eq.~\eqref{eq:iff} is equivalent to $n_i \ge t_i$. In other words, a player $i$ decides to invest \textit{iff} it is connected to at least $t_i$ investors.  To compute $t_i$, we first arrange the values of $\Delta g_i(n_i)$  as a non-decreasing sequence. Then we use a binary search to find the $n$ such that $\Delta g_i(n) \ge c_i$, which costs $O(\log{N})$ time. Finally we let $t_i=n$. 

We can think $t_i$ as a threshold. For a player $i$, no matter what the functional form of its utility function is, it invests \textit{iff} it has $t_i$ investing neighbors. Therefore we can use the payoff matrix in Table~\ref{tab:comple} to characterize the  utility function of player $i$ in a sense that the payoff matrix leads to the same decision as what the utility function leads to. The utility functions defined by Table~\ref{tab:comple} satisfy the \textit{increasing differences} property, which makes the associated functions $\hat{g}_i$ convex. In addition, the utility functions satisfy the non-decreasing assumption we made in Section~\ref{sec:model}. 
\begin{table}[h!]
\centering
\begin{tabular}{lccll}
                       & $n_i \ge t_i$               & $n_i < t_i$                &  &  \\ \cline{2-3}
\multicolumn{1}{l|}{0} & \multicolumn{1}{c|}{$c$} & \multicolumn{1}{c|}{$\gamma$} &  &  \\ \cline{2-3}
\multicolumn{1}{l|}{1} & \multicolumn{1}{c|}{$c+\gamma$} & \multicolumn{1}{c|}{0} &  &  \\ \cline{2-3}
                       &                         &                        &  & 
\end{tabular}
\caption{Payoff matrix of player $i$, where $c, \gamma > 0$ and $c \ge \gamma$. }
\label{tab:comple}
\end{table}

% \begin{equation}
% \begin{aligned}
% x_i = \begin{cases}1, & n_i>0 \\ 0, & n_i=0. \end{cases}
% \end{aligned}
% \label{eq:BR_comple}
% \end{equation}


Our problem  becomes tractable when $\hat{g}_i$ are convex, which is stated in  the following proposition:
\begin{proposition}\label{prop:comple}
When $\hat{g}_i$ is a convex function, the problem in Definition~\ref{def:main} can be solved in polynomial time.
\end{proposition}
\begin{proof}
It takes $O( N\log{N})$ to compute the threshold $t_i$ for every player.  In what follows we consider three special cases of $\bm{x}^{\ast}$, which cost at most $O(N)$ to determine if they are realizable. The special cases are $\bm{x}^{\ast} = \bm{1}$, $\bm{0}$ and $\sum_{i}^{}{x^{\ast}_i}= 1$. We  determine if the budget is enough to realize each case by iteratively checking if Eq.~\eqref{eq:iff} holds (not holds) for every investor (non-investor).


Suppose $\bm{x}^{\ast} \ne \bm{1}$, $\bm{0}$, and $\sum_{i}^{}{x^{\ast}_i}> 1$.  Let $\mathcal{S}^\prime:=\{i | x^{\ast}_i=0 \}$ be the set of non-investors. Similarly, let $\mathcal{S}:=\{ i | x^{\ast}_i=1 \}$ be those who invest. Suppose $t_i \le |\mathcal{S}|-1, \forall i \in \mathcal{S}$, otherwise we immediately conclude $\bm{x}^{\ast}$ is not realizable. 

The first step is to  remove edges such that each player $i \in \mathcal{S}^\prime$ have less than $t_i$ investing neighbors. Suppose the budget $B_1$ is enough to do so,  otherwise we conclude $\bm{x}^{\ast}$ is not realizable. This step costs $O(N)$. The second step is to check if we can make each player $i \in \mathcal{S}$ have investing neighbors greater than or equal to $t_i$. Define a set $\mathcal{S}_1 := \{ i \in \mathcal{S} | n_i < t_i \}$. Intuitively, $\mathcal{S}_1$ consists of those players that should invest in the target action profile but have less investing neighbors than their thresholds. If $|\mathcal{S}_1|=0$ we conclude $\bm{x}^{\ast}$ is realizable. Suppose $|\mathcal{S}_1| > 0$.  Let $\Delta = \{ \delta_i | \delta_i = t_i - n_i, \forall i \in \mathcal{S}_1 \}$, where each $\delta_i \in \Delta$ indicates how many extra investing neighbors player $i$ needs in order to invest. Let $\delta_{max}$ be the maximum of $\Delta$. We need to add at least $\delta_{max}$ edges. So if $B_1 < \delta_{max}$ we know $\bm{x}^{\ast}$ is not realizable. Suppose $B_1 \ge \delta_{max}$. To make $\bm{x}^{\ast}$ realizable, we need to let each $\delta_i \in \Delta$ reduce to zero. There are two strategies to reduce $\delta_i$. The first is to add an edge to $\mathcal{S}_1$, for example $(v, w)$ where $v, w \in \mathcal{S}_1$, which reduces $\delta_v$ and $\delta_w$ by one, respectively. The second is to add an edge between a player $i \in \mathcal{S}_1$ and another player $j \in \mathcal{S} \setminus \mathcal{S}_1$ (when $\mathcal{S} \setminus \mathcal{S}_1$ is not empty), which reduces $\delta_i$ by one. In order to implement the first strategy there needs to be at least a pair  of disconnected players in $\mathcal{S}_1$, which is captured by the condition in line 10 of Algorithm~\ref{algo:needed_edge}. Line 10-20 implements the first strategy. The second strategy (line 21-31) follows the implementation of the first one. To implement the second strategy to reduce, for example $\delta_i$, to zero, we pick any player $j \in \mathcal{S}\setminus \mathcal{S}_1$ such that $i$ and $j$ are  not connected, and add an edge between them. Note that we must be able to pick such a player $j$ from $\mathcal{S}\setminus \mathcal{S}_1$, otherwise player $i$ had $|\mathcal{S}|-1$ investing neighbors and it should have invested (recall the second strategy follows the implementation of the first one). 

Next, we show that \texttt{MinEdge} displayed in Algorithm~\ref{algo:needed_edge} finds the minimum number of edges to add. Let $T = \sum_{i \in \mathcal{S}_1}^{}{\delta_i}$. We need to reduce $T$ to zero.  Although there are two strategies to reduce $T$, the first strategy is more efficient than the second one in the sense that each edge added by the first strategy can reduce $T$ by two, while each edge added by the second strategy can only reduce $T$ by one. Line 10-20 of \texttt{MinEdge}  exploits the maximum number of edges that can be added by the first strategy, otherwise the \texttt{while-loop} would not terminate. \texttt{MinEdge} adds $\bar{a}$ edges using the first strategy, and $b$ edges using the second one. Suppose there is another algorithm that adds $a^\prime$ and $b^\prime$ edges using the first and the second strategy, respectively. Since:
\[
2\bar{a} + b = T = 2a^\prime + b \text{ and } \bar{a} \ge a.
\]
We conclude $\bar{a} + b \le a^\prime + b^\prime$, which shows that \texttt{MinEdge} adds the minimum number of edges. Line 10-20 costs $O(N)$, since the maximum number of edges that can be added by the first strategy is:
\[
\floor{ \frac{T}{2} } = \floor{ \frac{ \sum_{i\in \mathcal{S}_1}^{}{\delta_i} }{2} } \le \floor{ \frac{\bar{\delta}}{2} } \cdot |\mathcal{S}_1| = O(N),
\]
where $\bar{\delta} \ge \delta_i, \forall i$. Other operations of \texttt{MinEdge} cost at most $O(N)$. Finally, let $K$ be the number returned by \texttt{MinEdge}. We conclude $\bm{x}^{\ast}$ is realizable if $B_2 \ge K$.
\begin{algorithm}[h] 
\caption{MinEdge}\label{algo:needed_edge}
\begin{algorithmic}[1]
\State \textbf{Input}: $\mathcal{S}_1$ and its induced subgraph $\mathcal{G}_{\mathcal{S}_1}$
		\If{$\mathcal{S}_1=\{ k \}$}
			\State \textbf{Return} $\delta_k$
		\EndIf
		\If{$\mathcal{G}_{\mathcal{S}_1}$ is a clique}
				\State \textbf{Return} $\sum_{i\in \mathcal{S}_1}^{}{\delta_i}$
		\EndIf
		\State $K = 0$
		\State $D$ is an array: $D[i]=\delta_i, \forall i \in \mathcal{S}_1$
		\While{$\mathcal{G}_{\mathcal{S}_1}$ not a clique}
			\State Pick $i, j \in \mathcal{S}_1$, where $i, j$ not connected
			\State $D[i] = D[i] - 1, D[j] = D[j] - 1$
			\State $K = K+1$
			\If{$D[i]=0$}
				\State $\mathcal{S}_1 = \mathcal{S}_1 \setminus \{ i \}$
			\EndIf
			\If{$D[j]=0$}
				\State $\mathcal{S}_1 = \mathcal{S}_1 \setminus \{ j \}$
			\EndIf
		\EndWhile
		\If{$|\mathcal{S}_1|=0$}
			\State \textbf{Return} $K$
		\EndIf
		\If{$|\mathcal{S}_1|=1$}
			\State $K = K + D[k]$, where $k \in \mathcal{S}_1$
			\State \textbf{Return} $K$
		\EndIf
		\If{$|\mathcal{S}_1|>1$}
			\State $K = K + \sum_{i \in \mathcal{S}_1}^{}{D[i]}$
			\State \textbf{Return} $K$
		\EndIf
\end{algorithmic}
\end{algorithm}
\end{proof}

\subsection{Concave $\hat{g}_i$}
The analysis for the case where $g_i$ is a  concave function is similar to the one  for convex $g_i$. In particular, a player decides to invest \textit{iff} Eq.~\eqref{eq:iff} holds. Since $g_i$ are concave, $\Delta g_i(n_i)$ is non-increasing with respect to $n_i$. Therefore Eq.~\eqref{eq:iff} is equivalent to $n_i \le t_i$, which means a player $i$ decides to invest \textit{iff} the number of its investing neighbors is no larger than $t_i$. As we described in last section, $t_i$ can be thought as a threshold.   It takes $O(\log{N})$ to compute the threshold for each player. We use the payoff matrix in Table~\ref{tab:subs} to characterize the utility function of any player $i$. Note that the payoff matrix leads to the same decision for player $i$ as what its utility function leads to. The functions $\hat{g}_i$ associated with the utility functions defined by Table~\ref{tab:subs} are  concave. In addition, they are non-decreasing with respect to their arguments. 
\begin{table}[h!]
\centering
\begin{tabular}{lccll}
                       & $n_i > t_i$               & $n_i \le t_i$                &  &  \\ \cline{2-3}
\multicolumn{1}{l|}{0} & \multicolumn{1}{c|}{$c+\gamma$} & \multicolumn{1}{c|}{$0$} &  &  \\ \cline{2-3}
\multicolumn{1}{l|}{1} & \multicolumn{1}{c|}{$c$} & \multicolumn{1}{c|}{$\gamma$} &  &  \\ \cline{2-3}
                       &                         &                        &  & 
\end{tabular}
\caption{Payoff matrix of player $i$, where $c, \gamma > 0$ and $c \ge \gamma$.}
\label{tab:subs}
\end{table}


Our problem becomes tractable when $\hat{g}_i$ are concave:
\begin{proposition}\label{prop:subs}
When $\hat{g}_i$ is a concave function, the problem in Definition~\ref{def:main} can be solved in polynomial time. 
\end{proposition}
\begin{proof}
It takes $O( N\log{N})$ to compute the threshold $t_i$ for every player $i$.  In what follows we consider three special cases of $\bm{x}^{\ast}$, which cost at most $O(N)$ to determine if they are realizable. The special cases are $\bm{x}^{\ast} = \bm{1}$, $\bm{0}$ and $\sum_{i}^{}{x^{\ast}_i}= 1$. We  determine if our budget is enough to realize each case by iteratively checking if Eq.~\eqref{eq:iff} holds (not holds) for every investor (non-investor).

Suppose $\bm{x}^{\ast} \ne \bm{1}$, $\bm{0}$, and $\sum_{i}^{}{x^{\ast}_i}> 1$. We use $\mathcal{S}$ and $\mathcal{S}^\prime$ to denote the investing and non-investing players in $\bm{x}^{\ast}$, respectively.  The first step is to check if we have enough budget to add edges such that each player $i \in \mathcal{S}^\prime$ has more than $t_i$ investing neighbors.  This step takes $O(N)$ time. The second step is to let each player $i \in \mathcal{S}$ have at most $t_i$ investing neighbors. Let $\mathcal{S}_1:=\{ n_i > t_i | i \in \mathcal{S} \}$, which consist of those players that should invest in the target action profile but have investing neighbors more than their thresholds. If $|\mathcal{S}_1| = 0$ then $\bm{x}^{\ast}$ is realizable. Suppose $|\mathcal{S}_1| > 0$. Let $\Delta = \{ \delta_i | \delta_i = n_i - t_i, \forall i \in \mathcal{S}_1 \}$, where each $\delta_i \in \Delta$ indicates how many investing neighbors of player $i$ needs to be removed. Let $\delta_{max}$ be the maximum of $\Delta$. The budget to remove edges needs  to be at least $\delta_{max}$. Suppose $B_1 \ge \delta_{max}$, otherwise $\bm{x}^{\ast}$ is not realizable. To realize $\bm{x}^{\ast}$ we need to reduce each $\delta_i \in \Delta$ to zero. Similar to the analysis presented in the proof of Proposition~\ref{prop:comple},  there are also two strategies to reduce $\delta_i$. The first is to remove an edge from $\mathcal{S}_1$, for example removing $(v, w)$ where $v, w \in \mathcal{S}_1$, reduces $\delta_v$ and $\delta_w$ by one, respectively. The second is to remove an edge between a player $i \in \mathcal{S}_1$ and another player $j \in \mathcal{S} \setminus \mathcal{S}_1$ (when $\mathcal{S} \setminus \mathcal{S}_1$ is not empty), which reduces $\delta_i$ by one.  Let $\bar{\mathcal{G}}$ be the complement of $\mathcal{G}$ and $\bar{\mathcal{G}}_{\mathcal{S}_1}$ be the induced subgraph of $\mathcal{S}_1$ on $\bar{\mathcal{G}}$. Notice that removing an edge from $\mathcal{G}$ is equivalent to adding the edge to $\bar{\mathcal{G}}$. This indicates that we  can apply Algorithm~\ref{algo:needed_edge} on $\mathcal{S}_1$ and $\bar{\mathcal{G}}_{\mathcal{S}_1}$ to find the minimum number of edges to remove. Other analysis follows directly from the proof of Proposition~\ref{prop:comple}. 
\end{proof}




==> section/prob.tex <==
We consider a  Binary Networked Public Goods game (henceforth BNPG game). The BNPG is characterized by an undirected and connected graph $\mathcal{G}=(V, E)$ where the node set $V = \{1,2,\cdots,n\}$ denotes the players and $E = \{(i,j)|i,j \in V\}$ represents the interdependencies among the player's payoffs, a binary strategy space $x_i \in \{0,1\}$ for each player $i$ (we can think of these as decisions whether to \emph{invest in a public good}), and a collection of cost functions (negative utilities) $L_i(x_1,\ldots,x_n)$. These cost functions have special structures, which we now describe. We use a running example of crime reporting to illustrate the intuition behind this structure. 

Let $\mathcal{N}_i= \{ j  | (j, i) \in E \land j \ne i \}$ represent the set of neighbors of $i$, and define $n_i=\sum_{j \in \mathcal{N}_i}^{}{x_j}$ as the number of $i$'s neighbors who choose to invest. Thus, in the crime reporting scenario, $n_i$ is the number of $i$'s neighbors who report crimes. We assume that each player gains whenever more people invest (report crimes), for example, because as a result crime rate drops.
On the other hand, reporting crime is costly.
We capture the latter feature by introducing a cost $c_i$ which is incurred whenever $i$  invests in a public good.
Player $i$'s cost function is then defined as
\begin{eqnarray}
\label{eq:cost}
L_i(x_i,n_i) = c_i x_i + \lambda_i g_i(x_i + n_i),
\end{eqnarray}
where $g_i(x_i + n_i) \ge 0$ captures the positive externality of investment choices by $i$'s neighbors, such as the benefits to an individual when their neighbors report crimes, and $\lambda_i$ is a scaling factor representing the relative importance of the second term for a player's cost function.
The only restriction we impose on $g_i(\cdot)$ at this point is that they are \emph{decreasing} functions (e.g., higher reporting reduces crime rate).
Observe that the size of BNPG representation is $O(n^2)$ for an arbitrary $g_i(\cdot)$.


An action profile of the game is defined as: $\bm{x}=(x_1, \dots, x_n)$. Additionally,  let $\bm{x}_{-i}$ denote the joint actions of all the players other than player $i$. An approximate \emph{pure-strategy} Nash Equilibrium (PSNE) is defined as follow:	
\begin{defn}
	In a BNPG game an $\epsilon$-PSNE is a vector $\bm{x}=(x_1, \cdots, x_n) \in \{0, 1 \}^n$ such that:
	$$L_i(x_i, n_{i}) \le L_i(x^{\prime}_i, n_{i}) + \epsilon,$$
	$\forall i\in \{1, 2, \cdots, n \}$, where $n_i = \sum_{j\in \mathcal{N}_i} x_j$ and $0 \le \epsilon \le 1$.
\end{defn}


Given a graph $\mathcal{G}=(V, E)$, we would like to add or remove a set of edges such that a desired target action profile is an exact PSNE of the BNPG played on the resulted graph. We use a set $\mathcal{X}$ to characterize all the desired action profiles. For example, if our goal is to let \emph{k player invests}  then  the target class is defined as $\mathcal{X} :=\big\{\bm{x}^\ast | \sum_{i=1}^{}{x^{\ast}_i}=k \big\}$.

% a class of action profiles are $\epsilon$-PSNE of the BNPG played on the resulting graph. For example, we may want to add/remove a set of edges such that there are $k$ players invest.   Formally, the class of action profiles is termed target class and defined as a set $\mathcal{X}$. We add constraints to $\mathcal{X}$ to characterize a certain type of action profiles we want on the BNPG, for example, if our goal is to let \emph{k player invests}  then  the target class is defined as $\mathcal{X} :=\big\{\bm{x}^\ast | \sum_{i=1}^{}{x^{\ast}_i}=k \big\}$. 

==> section/set_utility.tex <==

Suppose we are given a specific target action profile $\bm{x}^{\ast}$. The formal definition of our problem is in Definition~\ref{def:given_profile}. Let $\mathcal{S}$ and $\mathcal{S}^\prime$ be the set of investors and non-investors, respectively. Define $\mathcal{S}_i = \mathcal{S} \cap \mathcal{N}_i$. Intuitively, $\mathcal{S}_i$ is the set of investors among the neighbors of player $i$. We define set-based utility functions as the following:
\begin{equation}\label{eq:set_utility}
\begin{aligned}
U_i(x_i, \mathcal{S}_i) = g_i(x_i, \mathcal{S}_i) - c_i x_i,
\end{aligned}
\end{equation}
where $g_i(x_i, \mathcal{S}_i) = \begin{cases} \hat{g}_i(\mathcal{S}_i \cup \{i \}), &  x_i = 1 \\ \hat{g}_i(\mathcal{S}_i), & x_i = 0 \end{cases}$, and $\hat{g}_i$ is a monotone sub/super-modular function. Note that the utility function defined in Eq.~\eqref{eq:utility} is a special cases of Eq.~\eqref{eq:set_utility} when $\hat{g}_i$ returns the cardinality of its argument. Similar to the analysis presented in last section, the sufficient and necessary condition for a player $i$ to invest is the following:
\begin{equation}\label{eq:iff_sub}
\underbrace{\hat{g}_i(\mathcal{S}_i \cup \{i \}) - \hat{g}_i(\mathcal{S}_i)}_{:=\Delta \hat{g}_i(\mathcal{S}_i)} \ge c_i.
\end{equation}
In what follows, we first show that it is NP-Complete to solve our problem when $\hat{g}_i$ are monotone submodular functions. The general idea is to construct a reduction from the \textit{Max-k-cover} problem. Then we the similar idea to show that our problem is also hard when $\hat{g}_i$ are monotone supermodular functions. 

\subsection{Submodular $\hat{g}_i$}
Since $\hat{g}_i$ is submodular, $\Delta \hat{g}_i(\mathcal{S}_i)$ is also a submodular function. In addition, $\Delta \hat{g}_i(\mathcal{S}_i)$ is non-increasing. Solving our problem is equivalent to  make  Eq.~\eqref{eq:iff_sub} hold for every investor, and not hold for every non-investor. In Theorem~\ref{th:submodular_hard} we prove that this is NP-Complete by a reduction from the \textit{Max-k-cover} problem. 

\begin{theorem}\label{th:submodular_hard}
When $\hat{g}_i$ are monotone submodular functions, the problem in Definition~\ref{def:given_profile} is NP-Complete. 
\end{theorem} 
\begin{proof}
First, given a target action profile $\bm{x}^{\ast}$ we can check if it is a PSNE by iteratively applying Eq.~\eqref{eq:iff_sub} to each player, which takes polynomial time. Next, we construct a reduction from the \textit{Max-k-cover} problem. Given a ground set $\mathcal{U}$, a set of subsets $\mathcal{A} = \{ A_1, A_2, \dots, A_m \,|\, \forall i: A_i\subseteq \mathcal{U} \}$, and an integer $k$, the objective of the \textit{Max-k-cover} problem is to find a subset $\mathcal{A}^\prime \subseteq \mathcal{A}$ such that $|\mathcal{A}^\prime| \le k$ and the number of covered elements $\big| \cup_{A_i \in \mathcal{A}^\prime} A_i \big|$ is maximized. We consider the decision version of the \textit{Max-k-cover} problem. Given an integer $m$, the decision version is to determine if the number of covered elements is at least $m$. For any instance  $MaxK(m)$  of the \textit{Max-k-cover} problem we construct an instance of our problem. The first step is to construct a graph $\mathcal{G}=(V, E)$. The node set $V$ consists of $m$ blue nodes and one red node, where each blue node corresponds to a set in $\mathcal{A}$. The edge set $E$ is empty. An example graph with $m=7$ is showed in Figure~\ref{fig:star_graph}. Next, we define the utility functions of the nodes. For blue nodes we set the  $\hat{g}_i$ associated with their utility functions as the following submodular function:
\[
\hat{g}_i(X) = |X|,
\]
which returns the cardinality of its argument. In addition, let the cost coefficients of all  blue nodes satisfy $c_i < 1$.  It is direct to verify that blue nodes always invest.  Notice that Eq.~\eqref{eq:iff_sub} is all we need to determine if a node invests. So for the red node $r$ we define the following:
\begin{equation}\label{eq:sub_g}
\Delta \hat{g}_r(\mathcal{S}_r) := \big| \cup_{i \in \mathcal{S}_r} A_i \big|,
\end{equation}
where $\mathcal{S}_r$ is the investors among the red node's neighbors.  The cost coefficient of the red node is set to $c_r=m$, so it invests \textit{iff} $\Delta \hat{g}_r(\mathcal{S}_r) \ge m$.  The budget parameters  are set to $B_1=0$ and $B_2 = k$, which means we can add at most $k$ edges but cannot remove any edge. We have $| \mathcal{S}_r | \le k$.
Suppose the target action profile $\bm{x}^{\ast} = \bm{1}$. Since the blue nodes always invest, what remains is to add edges such that the red node invests. If $\bm{x}^\ast$ is realizable,  then the answer to $MaxK(m)$ is ``yes''. Otherwise the answer is ``no''. Therefore if there were a polynomial-time algorithm to solve our problem, then the \textit{Max-k-cover} problem would be polynomial-time solvable. 

\begin{figure}[h]
\centering
\setlength{\tabcolsep}{0.1pt}
\begin{tabular}{c}
\stargraph{7}{2}
\end{tabular}
\caption{An example graph where each blue node corresponds to a set in $\mathcal{A}=\{A_1, \dots, A_7 \}$.}
\label{fig:star_graph}
\end{figure}
\end{proof}

\subsection{Supermodular $\hat{g}_i$}
When $\hat{g}_i$ are monotone supermodular functions our problem is still hard. The formal statement is in Theorem~\ref{th:supermodular_hard}. 
\begin{theorem}\label{th:supermodular_hard}
When $\hat{g}_i$ are monotone supermodular functions, the problem in Definition~\ref{def:given_profile} is NP-Complete. 
\end{theorem}
\begin{proof}
Given a target action profile $\bm{x}^{\ast}$ it takes polynomial time to check if it is a PSNE. Next, we utilize a  similar reduction  from the \textit{Max-k-cover} problem as presented in the proof of Theorem~\ref{th:submodular_hard}.  Given a ground set $\mathcal{U}$, a set of subsets $\mathcal{A} = \{ A_1, A_2, \dots, A_m \,|\, \forall i: A_i\subseteq \mathcal{U} \}$, and an integer $k$, the objective of the \textit{Max-k-cover} problem is to find a subset $\mathcal{A}^\prime \subseteq \mathcal{A}$ such that $|\mathcal{A}^\prime| \le k$ and the number of covered elements $\big| \cup_{A_i \in \mathcal{A}^\prime} A_i \big|$ is maximized. Given an integer $m$, the decision version is to decide if the number of covered elements is at least $m$.  Suppose we are given an instance $MaxK(m)$ of the decision version of \textit{Max-k-cover} problem, we construct a graph $\mathcal{G}=(V, E)$, where $V$ consists of $m$ blue nodes and one red node, and $E$ is an empty set. Each blue node corresponds to a set in $\mathcal{A}$. An example graph with $m=7$ is showed in Figure~\ref{fig:star_graph}.  Consider a target action profile $\bm{x}^{\ast}$ where all blue nodes invest and the red node does not invest. The utility functions of the blue nodes are the same as what we defined in the proof of Theorem~\ref{th:submodular_hard}, which makes the blue nodes always invest. The red node $r$ does not invest \textit{iff}:
\begin{equation}\label{eq:sup_g}
\Delta \hat{g}_r(\mathcal{S}_r) < c_r,
\end{equation}
where $\mathcal{S}_r$ is the investors among the red node's neighbors and $c_r$ is its cost coefficient. Eq.~\eqref{eq:sup_g} is equivalent to the following:
\[
\underbrace{-\Delta \hat{g}_i(\mathcal{S}_r) + \Delta \hat{g}_i(\mathcal{N}_i)}_{:=f(\mathcal{S}_r)} > \underbrace{- c_r +  \Delta \hat{g}_i(\mathcal{N}_i)}_{:=c^{\prime}_r},
\]
where $\mathcal{N}_r$ is the set of the red node's neighbors. Note that $\Delta \hat{g}_i$ is a non-decreasing function by the supermodularity of $\hat{g}_i$. Therefore $-\Delta \hat{g}_i(\mathcal{S}_r) + \Delta \hat{g}_i(\mathcal{N}_r) \ge 0$ since $\mathcal{S}_r \subseteq \mathcal{N}_r$. In addition, we have  $c^{\prime}_r=- c_r +  \Delta \hat{g}_i(\mathcal{N}_i) \ge 0$, otherwise the red node would always prefer not investing. The budget parameters are set to $B_1 = 0$ and $B_2 = k$, which means we can add up to $k$ edges but cannot remove any edge. We let $c^{\prime}_r=m-\epsilon$, where $\epsilon$ is a rational number and $0 < \epsilon < 1$. We define $f(\mathcal{S}_r)$ as the following:
\[
f(\mathcal{S}_r):= \big| \cup_{i \in \mathcal{S}_r} A_i \big|,
\]
where $|\mathcal{S}_r| \le k$. If $\bm{x}^{\ast}$ is realizable then $f(\mathcal{S}_r) > m - \epsilon$, which indicates the number of covered elements is at least $m$.  Therefore if there were a polynomial-time algorithm to determine if $\bm{x}^{\ast}$ is realizable, we would solve the \textit{Max-k-cover} problem in polynomial time. 
\end{proof}
